Highly unbreakable graph with a fixed excluded minor are almost rigid

A set $X \subseteq V(G)$ in a graph $G$ is $(q,k)$-unbreakable if every separation $(A,B)$ of order at most $k$ in $G$ satisfies $|A \cap X| \leq q$ or $|B \cap X| \leq q$. In this paper, we prove the following result: If a graph $G$ excludes a fixed complete graph $K_h$ as a minor and satisfies certain unbreakability guarantees, then $G$ is almost rigid in the following sense: the vertices of $G$ can be partitioned in an isomorphism-invariant way into a part inducing a graph of bounded treewidth and a part that admits a small isomorphism-invariant family of labelings. This result is the key ingredient in the fixed-parameter algorithm for Graph Isomorphism parameterized by the Hadwiger number of the graph, which is presented in a companion paper.

==> NE.tex <==
\input{NE-interface}

\subsection{Additional preliminaries}
\input{NE-prelims}

\subsection{Near-embeddings}
\input{NE-intro}

\subsubsection{Optimal near-embeddings}
\input{NE-optimal-near-embedding}

\subsection{Canonizing dongles}\label{ss:tidy-dongles}
\input{NE-tidy-dongles}

\subsection{Large grids}\label{ss:large-grids}
\input{NE-large-grids}

\subsection{Radial discs}\label{ss:radial-discs}
\input{NE-radial-discs}

\subsection{Universal apices}\label{ss:universal-apex}
\input{NE-universal-apex}

\subsection{Proximity of attachment points}\label{ss:proximity}
\input{NE-proximity}

\subsection{Wrap-up}
\input{NE-wrap-up}



